gatekeeper: Online Safety Verification and Control for Nonlinear Systems in Dynamic Environments

This paper presents the gatekeeper algorithm, a real-time and computationally-lightweight method that ensures that trajectories of a nonlinear system satisfy safety constraints despite sensing limitations. gatekeeper integrates with existing path planners and feedback controllers by introducing an additional verification step to ensure that proposed trajectories can be executed safely, despite nonlinear dynamics subject to bounded disturbances, input constraints and partial knowledge of the environment. Our key contribution is that (A) we propose an algorithm to recursively construct safe trajectories by numerically forward propagating the system over a (short) finite horizon, and (B) we prove that tracking such a trajectory ensures the system remains safe for all future time, i.e., beyond the finite horizon. We demonstrate the method in a simulation of a dynamic firefighting mission, and in physical experiments of a quadrotor navigating in an obstacle environment that is sensed online. We also provide comparisons against the state-of-the-art techniques for similar problems.

==> keywords.tex <==
% Collision Avoidance
% Motion and Path Planning
% Aerial Systems: Applications
% Sensor-based Control

  
%   	Aerial Systems: Applications
%  	Aerial Systems: Mechanics and Control
%  	Aerial Systems: Perception and Autonomy
%  	Autonomous Agents
%  	Autonomous Vehicle Navigation
%  	Collision Avoidance
%  	Motion and Path Planning
%  	Reactive and Sensor-Based Planning
%  	RGB-D Perception
%  	Visual-Based Navigation


%   	Additive Manufacturing
%  	Aerial Systems: Applications
%  	Aerial Systems: Mechanics and Control
%  	Aerial Systems: Perception and Autonomy
%  	Agent-Based Systems
%  	Agricultural Automation
%  	AI-Based Methods
%  	Assembly
%  	Automation at Micro-Nano Scales
%  	Automation in Life Sciences: Biotechnology, Pharmaceutical and Health Care
%  	Automation Technologies for Smart Cities
%  	Autonomous Agents
%  	Autonomous Vehicle Navigation
%  	Behavior-Based Systems
%  	Big Data in Robotics and Automation
%  	Biological Cell Manipulation
%  	Biologically-Inspired Robots
%  	Biomimetics
%  	Brain-Machine Interface
%  	Building Automation
%  	Calibration and Identification
%  	Cellular and Modular Robots
%  	Climbing Robots
%  	Cognitive Human-Robot Interaction
%  	Collision Avoidance
%  	Compliance and Impedance Control
%  	Compliant Assembly
%  	Compliant Joint/Mechanism
%  	Computational Geometry
%  	Computer Vision for Automation
%  	Computer Vision for Manufacturing
%  	Computer Vision for Medical Robotics
%  	Computer Vision for Other Robotic Applications
%  	Computer Vision for Transportation
%  	Contact Modeling
%  	Control Architectures and Programming
%  	Cooperating Robots
%  	Cooperative Manipulators
%  	Deep Learning in Robotics and Automation
%  	Demining Systems
%  	Dexterous Manipulation
%  	Direct/Inverse Dynamics Formulation
%  	Discrete Event Dynamic Automation Systems
%  	Distributed Robot Systems
%  	Domestic Robots
%  	Dual Arm Manipulation
%  	Dynamics
%  	Education Robotics
%  	Energy and Environment-Aware Automation
%  	Entertainment Robotics
%  	Environment Monitoring and Management
%  	Ethics and Philosophy
%  	Factory Automation
%  	Failure Detection and Recovery
%  	Field Robots
%  	Flexible Robots
%  	Force and Tactile Sensing
%  	Force Control
%  	Formal Methods in Robotics and Automation
%  	Foundations of Automation
%  	Gesture, Posture and Facial Expressions
%  	Grasping
%  	Grippers and Other End-Effectors
%  	Haptics and Haptic Interfaces
%  	Health Care Management
%  	Human Detection and Tracking
%  	Human Factors and Human-in-the-Loop
%  	Human Performance Augmentation
%  	Human-Centered Automation
%  	Human-Centered Robotics
%  	Humanoid and Bipedal Locomotion
%  	Humanoid Robots
%  	Hybrid Logical/Dynamical Planning and Verification
%  	Hydraulic/Pneumatic Actuators
%  	Industrial Robots
%  	Intelligent and Flexible Manufacturing
%  	Intelligent Transportation Systems
%  	Inventory Management
%  	Kinematics
%  	Learning and Adaptive Systems
%  	Learning from Demonstration
%  	Legged Robots
%  	Localization
%  	Logistics
%  	Manipulation Planning
%  	Manufacturing, Maintenance and Supply Chains
%  	Mapping
%  	Marine Robotics
%  	Mechanism Design
%  	Medical Robots and Systems
%  	Micro/Nano Robots
%  	Mining Robotics
%  	Mobile Manipulation
%  	Model Learning for Control
%  	Modeling, Control, and Learning for Soft Robots
%  	Motion and Path Planning
%  	Motion Control
%  	Motion Control of Manipulators
%  	Multi-Robot Systems
%  	Multifingered Hands
%  	Nanomanufacturing
%  	Natural Machine Motion
%  	Networked Robots
%  	Neural and Fuzzy Control
%  	Neurorobotics
%  	Nonholonomic Mechanisms and Systems
%  	Nonholonomic Motion Planning
%  	Object Detection, Segmentation and Categorization
%  	Omnidirectional Vision
%  	Optimization and Optimal Control
%  	Parallel Robots
%  	Passive Walking
%  	Path Planning for Multiple Mobile Robots or Agents
%  	Perception for Grasping and Manipulation
%  	Performance Evaluation and Benchmarking
%  	Petri Nets for Automation Control
%  	Physical Human-Robot Interaction
%  	Physically Assistive Devices
%  	Planning, Scheduling and Coordination
%  	Probability and Statistical Methods
%  	Process Control
%  	Product Design, Development and Prototyping
%  	Prosthetics and Exoskeletons
%  	Range Sensing
%  	Reactive and Sensor-Based Planning
%  	Recognition
%  	Redundant Robots
%  	Rehabilitation Robotics
%  	RGB-D Perception
%  	Robot Audition
%  	Robot Companions
%  	Robot Safety
%  	Robotics in Agriculture and Forestry
%  	Robotics in Construction
%  	Robotics in Hazardous Fields
%  	Robust/Adaptive Control of Robotic Systems
%  	Search and Rescue Robots
%  	Semantic Scene Understanding
%  	Semiconductor Manufacturing
%  	Sensor Fusion
%  	Sensor Networks
%  	Sensor-based Control
%  	Service Robots
%  	Simulation and Animation
%  	SLAM
%  	Social Human-Robot Interaction
%  	Soft Robot Applications
%  	Soft Robot Materials and Design
%  	Soft Sensors and Actuators
%  	Software, Middleware and Programming Environments
%  	Space Robotics and Automation
%  	Surgical Robotics: Laparoscopy
%  	Surgical Robotics: Planning
%  	Surgical Robotics: Steerable Catheters/Needles
%  	Surveillance Systems
%  	Sustainable Production and Service Automation
%  	Swarms
%  	Task Planning
%  	Telerobotics and Teleoperation
%  	Tendon/Wire Mechanism
%  	Underactuated Robots
%  	Virtual Reality and Interfaces
%  	Visual Learning
%  	Visual Servoing
%  	Visual Tracking
%  	Visual-Based Navigation
%  	Wearable Robots
%  	Wheeled Robots
